SpChar: Characterizing the Sparse Puzzle via Decision Trees

Sparse matrix computation is crucial in various modern applications, including large-scale graph analytics, deep learning, and recommender systems. The performance of sparse kernels varies greatly depending on the structure of the input matrix, making it difficult to gain a comprehensive understanding of sparse computation and its relationship to inputs, algorithms, and target machine architecture. Despite extensive research on certain sparse kernels, such as Sparse Matrix-Vector Multiplication (SpMV), the overall family of sparse algorithms has yet to be investigated as a whole. This paper introduces SpChar, a workload characterization methodology for general sparse computation. SpChar employs tree-based models to identify the most relevant hardware and input characteristics, starting from hardware and input-related metrics gathered from Performance Monitoring Counters (PMCs) and matrices. Our analysis enables the creation of a characterization loop that facilitates the optimization of sparse computation by mapping the impact of architectural features to inputs and algorithmic choices. We apply SpChar to more than 600 matrices from the SuiteSparse Matrix collection and three state-of-the-art Arm CPUs to determine the critical hardware and software characteristics that affect sparse computation. In our analysis, we determine that the biggest limiting factors for high-performance sparse computation are (1) the latency of the memory system, (2) the pipeline flush overhead resulting from branch misprediction, and (3) the poor reuse of cached elements. Additionally, we propose software and hardware optimizations that designers can implement to create a platform suitable for sparse computation. We then investigate these optimizations using the gem5 simulator to achieve a significant speedup of up to 2.63x compared to a CPU where the optimizations are not applied.

==> figures/reuse_distance.tex <==
%% TODO: redo

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figures/images/reuse_distance.pdf}
    \caption{Computing the reuse distance. The references array gets scanned linearly and, for each reference, we store the number of unique memory accesses that incur between two subsequent reference to that address. In our analysis, we use the average reuse distance per matrix.}
    \label{fig:reuse_distance}
\end{figure}

==> figures/reuse_index_distance.tex <==
%% TODO: redo

\begin{figure}
    \centering
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/reuse_distance.pdf}
        \caption{Reuse Distance}
        \label{fig:reuse_distance}
    \end{subfigure}%
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/images/index_distance.pdf}
        \caption{Index Distance}
        \label{fig:index_distance}
    \end{subfigure}
    \caption{For the reuse distance, the references array gets scanned linearly, and, for each reference, we store the number of unique memory accesses that incur between two subsequent references to that address. In our analysis. Similarly, for the index distance, we compute the difference in address for consecutive memory references. In our analysis, we use the average value as the main metric.}
\end{figure}


%Reuse Distance. The references array gets scanned linearly and, for each reference, we store the number of unique memory accesses that incur between two subsequent reference to that address. In our analysis, we use the average reuse distance per matrix.

==> plots/bias.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/images/fitted_vs_residuals.pdf}
    \caption{Normalized residuals (y axis) vs normalized predicted values (x axis).}
    \label{fig:bias}
\end{figure}

==> plots/mpki-spgemm.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/images/mpki-spgemm.pdf}
    \caption{\gls{mpki} for \spgemm{}. Lower cache size and shallower cache hierarchy leads to \postk{} having an order of magnitude more \gls{mpki} compared to \graviton{} and \kp{}.}
    \label{fig:mpki-spgemm}
\end{figure}

==> plots/performance-spgemm.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/images/performance-spgemm.pdf}
    \caption{Performance of \spgemm{} per \gls{cpu} and matrix category. \graviton achieves better performances thanks to the combination of bigger caches and wider \glspl{mshr} to both exploit the locality of the matrices and having multiple memory requests in flight when needed.}
    \label{fig:performance_spgemm}
\end{figure}

==> plots/r2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{plots/images/r2-all.png}
    \caption{$R^2$ for the normalized prediction (x axis) and true (y axis) values.}
    \label{fig:r2}
\end{figure}

==> plots/sim_bandwidth.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{plots/images/sim_bandwidth.pdf}
    \caption{Percentage of peak bandwidth utilized. Choosing the appropriate address mapping (\textbf{C3}) improves bandwidth utilization, whereas increasing the \glspl{mshr}' size (\textbf{C4}) yields diminishing returns.}
    \label{fig:sim_bandwidth}
\end{figure}


==> tables/real_world_matrix_metrics.tex <==
\begin{table}[]
    \centering
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|l|l|l|l|}
    \hline
        \textbf{Category} & \textbf{Temporal Locality} & \textbf{Spatial Locality} & \textbf{Row Imbalance} & \textbf{Branch Entropy} \\ \hline
        \textbf{2D/3D} & AVERAGE & HIGH & AVERAGE & LOW \\ 
        \textbf{Acoustics} & HIGH & HIGH & AVERAGE & LOW \\ 
        \textbf{Chemistry} & AVERAGE & AVERAGE & HIGH & HIGH \\ 
        \textbf{Circuits} & LOW & LOW & AVERAGE & AVERAGE \\ 
        \textbf{Computer Vision} & AVERAGE & AVERAGE & HIGH & LOW \\ 
        \textbf{Economy} & AVERAGE & HIGH & LOW & AVERAGE \\ 
        \textbf{Fluid Dynamics} & HIGH & HIGH & AVERAGE & AVERAGE \\ 
        \textbf{Graph} & LOW & LOW & HIGH & AVERAGE \\ 
        \textbf{Math} & AVERAGE & AVERAGE & AVERAGE & LOW \\ 
        \textbf{Physics} & HIGH & AVERAGE & LOW & AVERAGE \\ 
        \textbf{Semiconductors} & AVERAGE & AVERAGE & AVERAGE & HIGH \\ 
        \textbf{Structural} & HIGH & HIGH & AVERAGE & LOW \\ \hline
    \end{tabular}}
\end{table}
